An Empirical Study of Wrist-Target Construction and Joint-Angle Limits in Humanoid Arm Retargeting

Motion retargeting maps a demonstrated human movement onto a robot to compute its joint motion. This study examines how the construction of the desired wrist position affects whether computed arm joint angles reach their permitted limits on a Unitree H1-2. A reconstructed target is formed from demonstrated arm directions and robot segment lengths, so its shoulder-to-wrist distance depends on the demonstrated angle between the segments even when no posture-matching preference is applied. A reach-normalized target retains that direction while rescaling the distance, using the same processed demonstrations and the same joint-angle method. Across a forward-reach sweep the reconstructed target places a joint angle at a bound in 10 of 20 repetitions and the reach-normalized target in none. Across 25 recordings from one participant the corresponding counts are 8 and 6 on the reaching arm and 14 and 5 on the supporting arm, and a second participant repeats the bricklaying and lifting comparison. In hardware replay a joint is commanded to a bound in 12 of 16 direction-matching arm-records and in none of the 16 normalized records, and within the eligible records both tracking error and executed torque at those frames exceed their values elsewhere in the same run. Cross-body reach and arm-to-arm clearance identify limits of radial adjustment. The findings support treating target construction and posture matching as separate retargeting decisions, and evaluating both alongside the wrist positions and clearance that manipulation requires.

==> ieeeconf/tables/approach.tex <==
\begin{table}[!t]
\centering
\caption{Approach-direction contrast for the reconstructed target. The speed gate is a heuristic, not a ground-truth contact annotation. Counts use the provisional S1 25-capture summary.}
\label{tab:approach}
\small
\renewcommand{\arraystretch}{1.05}
\begin{tabular}{lcc}
\toprule
Activation & Reaching & Supporting \\
\midrule
No approach residual & 8/25 & 14/25 \\
Speed-gated residual & 19/25 & 13/25 \\
Always active & 23/25 & 13/25 \\
\bottomrule
\end{tabular}
\end{table}


==> ieeeconf/tables/factorial.tex <==
\begin{table}[!t]
\centering
\caption{Recorded saturation counts in the posture--centering study. Entries give reaching arm (supporting arm). S1 cohort inclusion remains provisional. Finite posture weights are soft preferences. Unverified normalized-margin values are not reproduced.}
\label{tab:factorial}
\small
\renewcommand{\arraystretch}{1.05}
\begin{tabular}{lcc}
\toprule
$w_l$ & Soft posture & No posture \\
\midrule
0 & 23/25 (15/25) & 10/25 (15/25) \\
0.05 & 16/25 (15/25) & 7/25 (12/25) \\
0.20$^{\dagger}$ & 6/25 (9/25) & 5/25 (8/25) \\
0.50$^{\dagger}$ & 0/25 (0/25) & 0/25 (0/25) \\
\bottomrule
\end{tabular}
\par\smallskip\begin{minipage}{0.97\columnwidth}\footnotesize
$^{\dagger}$ The recorded wrist-target errors at these weights are 40.4 and 149.9~mm. Their arm-by-posture assignment remains to be verified.
\end{minipage}
\end{table}


==> ieeeconf/tables/hardware.tex <==
\begin{table}[!t]
\centering
\caption{Position-derived replay summary. Correlations refer to 12 fidelity arm-runs and require final run-manifest verification. A no-saturation run has no defined conditional tracking ratio. Torque is not included because its signal provenance remains unresolved.}
\label{tab:hardware}
\small
\renewcommand{\arraystretch}{1.05}
\begin{tabular}{>{\raggedright\arraybackslash}p{0.67\columnwidth}r}
\toprule
Statistic & Recorded value \\
\midrule
Largest tracking ratios at two speeds & 1.89 / 1.79 \\
Corresponding saturated-frame fractions & 14\% / 12\% \\
Correlation with saturated-frame fraction & 0.850 \\
Correlation without one capture-arm at both speeds & 0.457 \\
Normalized replay: saturated command frames & 0 \\
\bottomrule
\end{tabular}
\end{table}


==> ieeeconf/tables/result_macros.tex <==
% Generated from data/project_log_summary.json. Counts are not raw-data-verified.
\newcommand{\MainRecReach}{8}
\newcommand{\MainRecSupport}{14}
\newcommand{\MainNormReach}{6}
\newcommand{\MainNormSupport}{5}
\newcommand{\FirstForwardRecReach}{2}
\newcommand{\FirstForwardRecSupport}{9}
\newcommand{\FirstForwardNormReach}{0}
\newcommand{\FirstForwardNormSupport}{1}
\newcommand{\SecondForwardRecReach}{2}
\newcommand{\SecondForwardRecSupport}{5}
\newcommand{\SecondForwardNormReach}{0}
\newcommand{\SecondForwardNormSupport}{1}


==> ieeeconf/tables/target_comparison.tex <==
\begin{table*}[!t]
\centering
\caption{Recorded target-definition results for both demonstrators. Entries give captures with commanded limit saturation on the reaching arm, with the supporting arm in parentheses. Direction matching and regularized direction retain posture commitments. Reconstructed and reach-normalized conditions remove the explicit posture term. The S1 pick-and-stack row and totals remain provisional because capture inclusion is unresolved.}
\label{tab:motions}
\small
\setlength{\tabcolsep}{8pt}
\renewcommand{\arraystretch}{1.05}
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{lcccc}
\toprule
Motion & Direction matching & Regularized direction & Reconstructed & Reach-normalized \\
\midrule
\multicolumn{5}{l}{\textit{S1: main motion comparison; reported five captures per motion}} \\
Overhead hammering & 0/5 (0/5) & 0/5 (0/5) & 0/5 (0/5) & 0/5 (0/5) \\
Bricklaying & 5/5 (5/5) & 5/5 (5/5) & 2/5 (5/5) & 0/5 (1/5) \\
Lifting & 5/5 (3/5) & 5/5 (4/5) & 0/5 (4/5) & 0/5 (0/5) \\
Pick-and-stack$^{\dagger}$ & 5/5 (5/5) & 2/5 (5/5) & 1/5 (5/5) & 1/5 (4/5) \\
Cross-body reach & 5/5 (0/5) & 5/5 (0/5) & 5/5 (0/5) & 5/5 (0/5) \\
\midrule
S1 total$^{\dagger}$ & 20/25 (13/25) & 17/25 (14/25) & 8/25 (14/25) & 6/25 (5/25) \\
\midrule
\multicolumn{5}{l}{\textit{S2: motion-level replication; five captures per motion}} \\
Bricklaying & 5/5 (5/5) & 4/5 (5/5) & 1/5 (4/5) & 0/5 (1/5) \\
Lifting & 5/5 (1/5) & 4/5 (0/5) & 1/5 (1/5) & 0/5 (0/5) \\
\midrule
S2 total & 10/10 (6/10) & 8/10 (5/10) & 2/10 (5/10) & 0/10 (1/10) \\
\bottomrule
\end{tabular}
\end{adjustbox}
\par\smallskip
\begin{minipage}{0.98\textwidth}\footnotesize
$^{\dagger}$ The result summary uses five pick-and-stack captures, whereas the acquisition notes list three clean captures. The original counts are retained without changing their denominators. The capture manifest must resolve this difference. Approach-residual settings also require confirmation across the main conditions.
\end{minipage}
\end{table*}

